Flavoured Dark Matter Moving Left

We investigate the phenomenology of a simplified model of flavoured Dark Matter (DM), with a dark fermionic flavour triplet coupling to the left-handed $SU(2)_L$ quark doublets via a scalar mediator. The DM-quark coupling matrix is assumed to constitute the only new source of flavour and CP violation, following the hypothesis of Dark Minimal Flavour Violation. We analyse the constraints from LHC searches, from meson mixing data in the $K$, $D$, and $B_{d,s}$ meson systems, from thermal DM freeze-out, and from direct detection experiments. Our combined analysis shows that while the experimental constraints are similar to the DMFV models with DM coupling to right-handed quarks, the multitude of couplings between DM and the SM quark sector resulting from the $SU(2)_L$ structure implies a richer phenomenology and significantly alters the resulting impact on the viable parameter space.

==> praeambel/befehle.tex <==
%Lösche voreingestellte Symbole
\savesymbol{a}
\savesymbol{b}
\savesymbol{d}
\savesymbol{e}
\savesymbol{gg}
\savesymbol{k}
\savesymbol{l}
\savesymbol{L}
\savesymbol{p}
\savesymbol{r}
\savesymbol{s}
\savesymbol{t}
\savesymbol{div}
\savesymbol{SS}



%Sprachen
\newcommand{\englisch}[1]{\begin{otherlanguage}{british}#1\end{otherlanguage}}
\newcommand{\deutsch}[1]{\begin{otherlanguage}{ngerman}#1\end{otherlanguage}}

%Textauszeichnung
\newcommand{\schlsswrt}[1]{\textbf{#1}}  %Schlüsselwort
\newcommand{\betont}[1]{\textsl{#1}} % Betonung

%Anzeigestil in Formeln
\newcommand{\D}{\displaystyle}

%Mathematische Funktionen
\DeclareMathOperator{\varRe}{Re}  %Realteil als Re
\DeclareMathOperator{\varIm}{Im}  %Imaginärteil als Im
\DeclareMathOperator{\arcsec}{arcsec} 
\DeclareMathOperator{\arccsc}{arccsc}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arccsch}
\DeclareMathOperator{\arccoth}{arccoth}

\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\div}{div}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\Gl}{GL}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\diag}{diag}
\newcommand{\ip}{\ \lrcorner\ }

%Mathematische Akzente
\newcommand{\konj}[1]{\overline{#1}}  % komplex Konjugiertes
\newcommand{\evec}[1]{\hat{#1}}  % Einheitsvektoren auszeichnen
\newcommand{\ten}[1]{\overleftrightarrow{#1}}	% Tensorzeichen

%Griechische Buchstaben und co
\newcommand{\a}{\alpha}
\newcommand{\b}{\beta}
\newcommand{\d}{\partial}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\e}{\varepsilon}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\k}{\kappa}
\newcommand{\l}{\lambda}
\newcommand{\L}{\Lambda}
\newcommand{\p}{\phi}
\newcommand{\ps}{\psi}
\newcommand{\r}{\rho}
\newcommand{\s}{\sigma}
\newcommand{\t}{\theta}
\newcommand{\A}{\mathcal A}
\newcommand{\Acl}{A_{cl}}
\newcommand{\B}{\mathbf B}

%Farben
\newcommand{\blue}[1]{\color{blue}#1\color{black}}
\newcommand{\red}[1]{\color{red}#1\color{black}}
\newcommand{\green}[1]{\color{green}#1\color{black}}


%Grenzwerte
\newcommand{\limes}[1]{\underset{#1}\lim}  %lim mit Argument darunter
\newcommand{\gw}[1]{\xrightarrow{#1}}  %Pfeil mit Argument darüber (Grenzwert)
\newcommand{\glmgw}[1]{\rightrightarrows} % gleichmäßiger Grenzwert

%Mengen
\newcommand{\N}{\mathbbm{N}}
\newcommand{\Z}{\mathbbm{Z}}
\newcommand{\Q}{\mathbbm{Q}}
\newcommand{\R}{\mathbbm{R}}
\newcommand{\Rpl}{\mathbbm{R}_+}
\newcommand{\Rmin}{\mathbbm{R}_-}
\newcommand{\C}{\mathbbm{C}}
\newcommand{\K}{\mathbbm{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\SS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\gg}{\mathbf g}


%Matrizen
\newcommand{\mat}[1]{\hat{#1}} % Akzent für Matrizen
\newcommand{\NullMatrix}{\textbf{0}}
\newcommand{\EinsMatrix}{\textbf{1}}

%Bra, Ket-Vaktoren
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{| #1 \rangle}

%Operatoren
\newcommand{\diff}[2]{\frac{\text{d}#1}{\text{d}#2}} %Ableitung nach Leibnitz geschrieben
\newcommand{\pdiff}[2]{\frac{\partial#1}{\partial #2}} %partielle Ableitung nach Leibnitz geschrieben
\newcommand{\laplace}{\Delta} % Laplace-Operator


%Einheiten
\usepackage{gensymb} % notwendiges Paket mit Symbolen
\newcommand{\Einheit}[1]{\,\text{#1}}
\newcommand{\Ampere}{\Einheit{A}}
\newcommand{\Sekunde}{\Einheit{s}}
\newcommand{\Gramm}{\Einheit{g}}
\newcommand{\Meter}{\Einheit{m}}
\newcommand{\Newton}{\Einheit{N}}
\newcommand{\Pascal}{\Einheit{Pa}}
\newcommand{\Farad}{\Einheit{F}}
\newcommand{\Volt}{\Einheit{V}}
\newcommand{\Coulomb}{\Einheit{C}}
\newcommand{\Joule}{\Einheit{J}}
\newcommand{\Tesla}{\Einheit{T}}
\newcommand{\Liter}{\Einheit{l}}
\newcommand{\Gauss}{\Einheit{G}}
\newcommand{\Ohm}{\,\ohm}
\newcommand{\Siemens}{\Einheit{S}}
\newcommand{\Henry}{\Einheit{H}}
\newcommand{\Watt}{\Einheit{W}}
\newcommand{\Hertz}{\Einheit{Hz}}
\newcommand{\Grad}{\degree}
\newcommand{\Celsius}{\,\celsius}
\newcommand{\Kelvin}{\Einheit{K}}
\newcommand{\varGrad}{\Einheit{grd}}
\newcommand{\EVolt}{\Einheit{eV}}
\newcommand{\Mol}{\Einheit{mol}}
\newcommand{\Skalenteil}{\Einheit{Skt}}
\newcommand{\Angstroem}{\Einheit{\AA}}

\newcommand{\rpm}{\Einheit{rpm}}
\newcommand{\dalton}{\Einheit{da}}
\newcommand{\molar}{\Einheit{M}}

\newcommand{\Yotta}{\Einheit{Y}\hspace{-0.5ex}}
\newcommand{\Zetta}{\Einheit{Z}\hspace{-0.5ex}}
\newcommand{\Exa}{\Einheit{E}\hspace{-0.5ex}}
\newcommand{\Peta}{\Einheit{P}\hspace{-0.5ex}}
\newcommand{\Tera}{\Einheit{T}\hspace{-0.5ex}}
\newcommand{\Giga}{\Einheit{G}\hspace{-0.5ex}}
\newcommand{\Mega}{\Einheit{M}\hspace{-0.5ex}}
\newcommand{\Kilo}{\Einheit{k}\hspace{-0.5ex}}
\newcommand{\Hekto}{\Einheit{h}\hspace{-0.5ex}}
\newcommand{\Deka}{\Einheit{da}\hspace{-0.5ex}}
\newcommand{\dezi}{\Einheit{d}\hspace{-0.5ex}}
\newcommand{\centi}{\Einheit{c}\hspace{-0.5ex}}
\newcommand{\milli}{\Einheit{m}\hspace{-0.5ex}}
\newcommand{\mikro}{\,\micro\hspace{-0.5ex}}
\newcommand{\nano}{\Einheit{n}\hspace{-0.5ex}}
\newcommand{\pico}{\Einheit{p}\hspace{-0.5ex}}
\newcommand{\femto}{\Einheit{f}\hspace{-0.5ex}}
\newcommand{\atto}{\Einheit{a}\hspace{-0.5ex}}
\newcommand{\zepto}{\Einheit{z}\hspace{-0.5ex}}
\newcommand{\yokto}{\Einheit{y}\hspace{-0.5ex}}


==> praeambel/makros.tex <==
%Leerraum statt Text einfügen
\newlength{\tmplen}
\newcommand{\leer}[1]{\settowidth{\tmplen}{#1}\hspace*{\tmplen}}
\newcommand{\nleer}[1]{\settowidth{\tmplen}{#1}\hspace*{-\tmplen}}

%Definitionsbox:
\newcommand{\mybox}[2]{
    \bigbreak
    \fcolorbox{black}{white}{\parbox{\linewidth}{
    	\textbf{#1} \\
    	#2}}
    \bigbreak
}


==> praeambel/pakete.tex <==
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc} %lege Latin1 als Eingabgeformat fest
\usepackage[ngerman,british]{babel} %lege Deutsch als Sprache fest, neue Rechtschreibung
	\addto\captionsngerman{\renewcommand{\figurename}{Abb.}\renewcommand{\tablename}{Tab.}} %eigene Kürzel für Abbildungen und Tabellen
\usepackage{amsmath} %AMS Mathematik-Pakte
\usepackage{amssymb} %AMS Symbol-Paket
\usepackage{mathrsfs} %Skript-Buchstaben
\usepackage{bbm} %für Mengenzeichen
\usepackage{mdwlist} %mehr Listenumgebungen
\usepackage{paralist} %mehr Listenumgebungen
	\setlength{\pltopsep}{0.5em} %Abstand zwischen Liste und umgebenden Text für paralist
	\setlength{\plitemsep}{0.3em} %Abstand zwischen Listenelementen für paralist
\usepackage{array}
\usepackage{graphicx} %zum Einbinden von Grafiken
\usepackage{booktabs} %stellt unterschiedlich dicke horizontale Trennlinien für Tabellen bereit
\usepackage{multirow} %zum Setzen von mehrspaltigen Zellen in Tabellen
\usepackage{multicol}
\usepackage{dcolumn} %zum Setzen reiner Zahlenspalten in Tabellen
\usepackage{wrapfig} %Umgebungen für textumflossene Grafiken
\usepackage{url} %stellt Umgebung zum Setzen von URL bereit
\usepackage{ziffer} %legt Komma statt Punkt als Trennzeichen in Dezimalbrüchen fest
\usepackage{scrpage2} %zu KOMA-Script kompatible Kopf- und Fußzeilen
\usepackage{color} %Unterstützung für Farbe
\usepackage[version=3]{mhchem} %für den Satz Chemischer Formeln
\usepackage{lscape} %Querformat-Umgebung

\usepackage{amsthm,dsfont,mathtools} % Weiteres Mathezeug
\usepackage{savesym} %Zum Überschreiben voreingestellter Befehle

%Für Feynmandiagramme:
\usepackage{latexsym}
\usepackage{feynmp}
